Prospects for Future Binary Black Hole GW Studies in Light of PTA Measurements

NANOGrav and other Pulsar Timing Arrays (PTAs) have discovered a common-spectrum process in the nHz range that may be due to gravitational waves (GWs): if so, they are likely to have been generated by black hole (BH) binaries with total masses $> 10^9 M_{\odot}$. Using the Extended Press-Schechter formalism to model the galactic halo mass function and a simple relation between the halo and BH masses suggests that these binaries have redshifts $z = {O}(1)$ and mass ratios $\gtrsim 10$, and that the GW signal at frequencies above ${O}(10)$~nHz may be dominated by relatively few binaries that could be distinguished experimentally and would yield observable circular polarization. Extrapolating the model to higher frequencies indicates that future GW detectors such as LISA and AEDGE could extend the PTA observations to lower BH masses $\in (10^6, 10^9 ) M_{\odot}$ and $\in (10^3, 10^9) M_{\odot}$.

==> reply.tex <==


We thank the Referee for the useful comments and suggestions. We will address all points raised by the Referee separately:

1. We included the missing references, added a new footnote one to address the alternative interpretation of quasar optical variability and a new footnote 3 to mention that the PTA binaries could not explain the quasi-periodicity in blazars.

2. We improved the readability of section 2 by rewriting the text between Eqs. (1) and (2). In particular, we added that $\delta_c(z)$ is the critical overdensity for collapse.

We changed the discussion below Eq. (4) to clarify that it is a problem of the EPS formalism that Q is not symmetric. Q is symmetric in the BKH formalism, and it was shown by Erickcek et al. that taking $M_1 < M_2$ in the EPS result approximates well the BKH result.

Regarding the z-dependence of $p_{\rm occ}$, we extended the discussion below Eq. (6) and added a comment on page 8. 

Referee Report

1. Introduction:

I suggest the authors extend the introduction with relevant references.

The authors report that “[…] observations of quasar optical variability provide indirect evidence for the existence of some tight [..]”.

Several observational and theoretical studies have shown that the periodic flux variation and periodic outburst activities in the radio, optical, X-ray, and &#947; -ray light curves is possibly associated to the orbital motion of a black hole binaries in the center of many galaxies. See e.g. Rieger et al., 2000, A&A, 359, 948, De Paolis, et al., A. A. 2002, A&A, 388, 470
De Paolis, et al., 2004, A&A, 426, 379, Iguchi et al., 2010, ApJ, 724, L166, Kovacevic et al., A&A 663, A99, 2022)

The authors could also cite alternative scenarios since quasi-periodic features may also be due to intrinsic variability in the accretion disc such as low-frequency quasi-periodic oscillations ( see e.g. King O. G. et al., 2013, MNRAS, 436, L114). Also self-lensing by an intrinsic population of stars could produce scintillation and variability (although on different time scales). And red noise could induce, in some cases, a wrong interpretation.

Note also that: the sources show quasi-periodic variability on year-like time scales and are possibly connected to massive black hole binaries to contribute to the nanohertz gravitational-wave stochastic background. But as shown by Holgado et al., MNRAS 481, L74–L78 (2018), binarity cannot significantly explain year-like quasi-periodicity in blazars.

2. Section 2:

I suggest improvements in the readability of the paper at some points. For example, in eq. 1 the authors introduce the halo mass function, which depends on several parameters among which $\delta_c(z)$. I think that introducing the correct units would help.

Can you give an explanation for why Q(M1.M2, t) is not symmetric in the exchange of M1 and M2? One would expect that the probability for M1 to merge with M2 and form Mf should be the same if the indices are swapped.

In equation 7, $p_{occ}(m_1)$ and $p_{occ}(m_2)$ do not depend on the redshift z. However, as shown for example by Lippi et al., ApJ, 2009, 701, 360 (but see also the relevant literature) the occupation fraction of the black hole binary might be a function of z. Could you comment? How would your results change if the fraction is allowed to vary with z according to a given law? The above authors find, for example, that a fraction between 0.1 and 1 reproduces well the observation.
